Matching-Based Selection with Incomplete Lists for Decomposition Multi-Objective Optimization

The balance between convergence and diversity is a key issue of evolutionary multi-objective optimization. The recently proposed stable matching-based selection provides a new perspective to handle this balance under the framework of decomposition multi-objective optimization. In particular, the stable matching between subproblems and solutions, which achieves an equilibrium between their mutual preferences, implicitly strikes a balance between the convergence and diversity. Nevertheless, the original stable matching model has a high risk of matching a solution with a unfavorable subproblem which finally leads to an imbalanced selection result. In this paper, we propose an adaptive two-level stable matching-based selection for decomposition multi-objective optimization. Specifically, borrowing the idea of stable matching with incomplete lists, we match each solution with one of its favorite subproblems by restricting the length of its preference list during the first-level stable matching. During the second-level stable matching, the remaining subproblems are thereafter matched with their favorite solutions according to the classic stable matching model. In particular, we develop an adaptive mechanism to automatically set the length of preference list for each solution according to its local competitiveness. The performance of our proposed method is validated and compared with several state-of-the-art evolutionary multi-objective optimization algorithms on 62 benchmark problem instances. Empirical results fully demonstrate the competitive performance of our proposed method on problems with complicated Pareto sets and those with more than three objectives.

==> algorithm.tex <==
% !Tex root = main.tex

\section{Proposed Algorithm: MOEA/D-ASTM}
\label{sec:algorithm}

In order to make use of our local competitiveness-based approach to set the length of solutions' preference lists, we propose the adaptive two-level stable matching-based selection and integrate it into MOEA/D-DRA framework. In this section, the proposed algorithm, referred as MOEA/D-ASTM is presented and its computational complexity is analyzed. Besides, MOEA/D-ASTM is compared with two MOEA/D variants with state-of-the-art environmental selection operator, i.e. gMOEA/D-AGR \cite{WangZZGJ16} and MOEA/D-IR \cite{LiKZD15}.

\subsection{Adaptive Two-Level Stable Matching-Based Selection}
The adaptive two-level stable matching-based selection is based on the original stable matching-based selection. Since the local competitiveness-based approach does not require a prior knowledge of the stable matching, it can be directly plugged into line 2 of \pref{alg:stm2l}. As presented in \pref{sec:stablematching}, $\Delta _X(\mathbf{x},p)$ is defined as the Euclidean distance between the normalized objective vector of $\mathbf{x}$ and the weight vector of $p$ in the objective space. But the objective vector of $\mathbf{x}$ in $\Delta _P(p,\mathbf{x})$ is not normalized in \cite{LiZKLW14}. To make $\Delta _P(p,\mathbf{x})$ coincident with $\Delta _X(\mathbf{x},p)$, $\Delta _P(p,\mathbf{x})$ is refined as
\begin{equation}
\Delta_P(p,\mathbf{x})=\max \limits_{1\leq i\leq m}\{|\overline{f}_i(\mathbf{x})|/w_i\}.
\label{eq:preference_p2}
\end{equation}
The normalization method proposed in \cite{DebJ14} is adopted.

\subsection{Comparisons with gMOEA/D-AGR and MOEA/D-IR}
MOEA/D-ASTM, gMOEA/D-AGR and MOEA/D-IR are all based on MOEA/D and conduct environmental selection on a generational basis. Since their main advancement is on the environmental selection operator, we only discuss the similarities and differences between their selection operators as follows.

\subsubsection{Similarities}
\begin{itemize}
\item All the three MOEAs employ the TCH aggregated objective of the subproblems to pursue convergence.
\item All the three MOEAs utilize the perpendicular distance between the objective vector of the solution and the weight vector of the subproblem to contribute to diversity.
%\item Both of MOEA/D-ASTM and gMOEA/D-AGR introduce a neighborhood concept to assist the selection.
\item Both of MOEA/D-ASTM and gMOEA/D-AGR adopt an adaptive approach to dynamically control the problem dependent parameter.
\item Both of MOEA/D-ASTM and MOEA/D-IR define the preferences between subproblems and solutions. The convergence and diversity is achieved by a selection fulfilling their preferences.
\end{itemize}

\subsubsection{Differences}
\begin{itemize}
\item The selection in MOEA/D-ASTM is modeled as an SMP with incomplete lists. The environmental selection are done by computing a stable matching between the subproblems and solutions, where the diversity is ensured by limiting the length of solutions' preference list. In contrast, gMOEA/D-AGR employs a replacement neighborhood of limited size to pursue diversity. Similarly, MOEA/D-IR defines a related set for a subproblem containing a limited number of closest solutions that prefer the subproblem. Furthermore, a niche count \cite{LiKZD15} is embedded into the definition of the preference of a solution on subproblems to help the diversity.
\item In MOEA/D-ASTM, a set of closest subproblems are collected for a solution to help measure the local competitiveness of each solution. Whereas in gMOEA/D-AGR, the replacement neighborhood is defined as a set of closest solutions for a subproblem, so that only solutions in the replacement neighborhood could update the current solution of the subproblem.
\item MOEA/D-ASTM proposes an adaptive approach to set the length of the preference list dynamically according to the real-time local competitiveness for different solutions. By contrast, gMOEA/D-AGR adopts a sigmoid function to dynamically control a same size of replacement neighborhood for all subproblems. However, different subproblems may require different extent of efforts on diversity. Therefore, simply determining a same replacement neighborhood size for all subproblems is undesired.
\end{itemize}

